Large-scale Reinforcement Learning for Diffusion Models

Text-to-image diffusion models are a class of deep generative models that have demonstrated an impressive capacity for high-quality image generation. However, these models are susceptible to implicit biases that arise from web-scale text-image training pairs and may inaccurately model aspects of images we care about. This can result in suboptimal samples, model bias, and images that do not align with human ethics and preferences. In this paper, we present an effective scalable algorithm to improve diffusion models using Reinforcement Learning (RL) across a diverse set of reward functions, such as human preference, compositionality, and fairness over millions of images. We illustrate how our approach substantially outperforms existing methods for aligning diffusion models with human preferences. We further illustrate how this substantially improves pretrained Stable Diffusion (SD) models, generating samples that are preferred by humans 80.3% of the time over those from the base SD model while simultaneously improving both the composition and diversity of generated samples.

==> sec/2_related_work_long_version.tex <==
\section{Related Work}
\label{sec:related_work}

\paragraph{Text-to-Image Diffusion Models.}
Denoising diffusion probabilistic models (DDPMs)~\cite{sohldickstein2015deep, ho2020denoising} have emerged as the de-facto standard for image generation, which utilize an iterative denoising process to transform Gaussian noise into images that follow a learned data distribution. Latent Diffusion Models (LDMs)~\cite{rombach2022highresolution} extend traditional DDPMs to operate in an image latent space instead of the pixel space by utilizing pretrained encoder-decoder models i.e. VAEs~\cite{kingma2022autoencoding}, allowing for improved efficiency and scalability. While diffusion models are trained by optimizing a variational lower bound on the log-likelihood of the data samples, in practice we may be interested in other aspects of the samples (e.g. human preferences or text-image alignment) rather than likelihoods. In this paper, we present a scalable RL framework on fine-tuning diffusion models optimizing for arbitrary downstream objectives. 
%\newline\newline
\paragraph{Learning Human Preferences.}
A number of works have studied using human feedback to align AI systems with human intent \cite{christiano2023deep, kreutzer2018neural, ziegler2020finetuning, stiennon2022learning, ouyang2022training, liu2023chain} by learning a reward function to reflect human preferences via human judgements of model outputs. In the language modeling community, reinforcement learning from human feedback (RLHF) \cite{ouyang2022training, nakano2022webgpt, bai2022training} has emerged as a powerful method to align large language models (LLMs) with human preferences and social values, by fine-tuning LLMs using RL methods like proximal policy optimization (PPO) ~\cite{schulman2017proximal}. In particular, InstructGPT \cite{ouyang2022training} significantly improved alignment for GPT-3 and built a strong foundation for the success of ChatGPT. Recent works have attempted to apply similar methods to text-to-image diffusion models, by training reward functions with large-scale expert annotation \cite{xu2023imagereward} or real users' choices on generated images \cite{kirstain2023pickapic, wu2023human}.
%\newline\newline

\paragraph{Reward Fine-tuning for Diffusion Models.} Existing reward fine-tuning methods for diffusion models can be classified into three categories: supervised, gradient-based or RL-based. Lee~\etal~\cite{lee2023aligning} and Wu~\etal \cite{wu2023human} proposed supervised approaches, both of which generate samples with a pre-trained diffusion model and use the generated images for fine-tuning the model, by either weighting the samples according to their reward values \cite{lee2023aligning} or prepending an identifier to the low-reward samples \cite{wu2023human}. Unlike online learning methods like RL, the samples are not generated with the current policy. Dong~\etal\cite{dong2023raft} proposed an online supervised fine-tuning method, where the policy used for sampling is updated in every iteration of training, and the images with the highest rewards are selected as training data for the next iteration. 

ReFL \cite{xu2023imagereward} and DRaFT \cite{clark2023directly} are gradient-based optimization algorithms that backpropagate the gradient through the reward model. ReFL evaluates the reward on the one-step predicted clean image from a random timestep along the denoising trajectory, and DRaFT backpropagates through the full sampling procedure. While the one-step prediction deviates from the actual distribution of the final sample images, backpropagation through multiple diffusion model calls imposes a heavy burden on the memory resource. In addition, many reward functions are not differentiable and thus these methods are not always applicable in practice.  

More recently, DDPO \cite{black2023training} and DPOK \cite{fan2023dpok} investigate into RL fine-tuning of diffusion models with policy gradient algorithms, formulating the optimization as a multi-step
decision-making problem. Both works have narrow scope in that DPOK uses a training set of 4 prompts only and mainly focus on training a separate model for each prompt, and DDPO uses a simple set of 45 common animals and 3 activities for their text-image alignment experiment and does not include human preference reward as training signal. In contrast, we aim to improve the general performance of state-of-the-art diffusion models on extensive and diverse prompts across different tasks. We perform multi-reward joint training with million-sized prompts to optimize SD models for human preferences, compositional capacities as well as diversity and fairness simultaneously. 

\paragraph{Compositional Text-to-image generation.} Despite their remarkable capacity, current state-of-the-art text-to-image models still struggle to generate images that faithfully align with the semantics of the text prompts due to their limited compositional capabilities~\cite{cho2023dalleval, gokhale2023benchmarking, huang2023t2icompbench}. For example, they often fail to effectively compose different objects into a complex and coherent scene, resulting in entity leakage, attribute leakage, and missing entities~\cite{wang2023compositional}. Several works such as Attend-and-Excite \cite{chefer2023attendandexcite}, Composable Diffusion \cite{liu2022compositional}, Structure Diffusion \cite{feng2023trainingfree} and Space-Time
Attention \cite{wu2023harnessing} propose to address these shortcomings post-hoc by
manipulating the inference process. While showcasing superior qualitative results, these approaches often result in a much more expensive generation process (with \cite{chefer2023attendandexcite} being around 6x slower and \cite{wu2023harnessing} over 100x \cite{karthik2023dont}). Another line of work strives to improve the controllability  by using auxiliary conditioning inputs such as bounding boxes \cite{chen2023trainingfree, li2023gligen} or spatial layouts \cite{wu2023harnessing,  lian2023llmgrounded, feng2023layoutgpt}. Our method instead focus on improving the fidelity of existing SD models without using additional layout guidance. 

\paragraph{Inclusive Text-to-Image Generation.}
Text-to-image generative models have the inherent flaw that they perpetuate and even amplify the societal biases present in the massive pretraining datasets of uncurated image-text pairs \cite{cho2023dalleval, zhang2023auditing, changpinyo2021conceptual,CheongManuscript-CHEIGA-2}. Recent works \cite{smith2023balancing, Bianchi_2023,luccioni2023stable} have revealed severe ethnic, racial, class, gendered, and inter-sectional stereotypes \cite{naik2023social} in state-of-the-art text-to-image models, including SD and Dall·E \cite{ramesh2022hierarchical}. Smith \etal propose to mitigate the bias in vision-language datasets with balanced synthetic data, utilizing an image editing pipeline. Along similar lines, Esposito ~\etal fine-tune text-to-image models with synthetic data that varies in perceived skin tones and genders. Several recent works have also proposed to instruct text-to-image diffusion models on fairness with textual guidance during inference \cite{friedrich2023fair} or with reference images of a particular attribute \cite{zhang2023inclusive}. Different from prior work, our method does not require synthetic data collection or inference-time intervention.


% For example, the authors of DALL-E Mini, acknowledge the limitation of their model ``Occupations demonstrating higher levels of education ...or high physical labor...are mostly represented by white men. In contrast, nurses, secretaries or assistants are typically women, often white as well 

==> tables/IM_baselines.tex <==
\def\thickhline{\noalign{\hrule height.8pt}}
      
\begin{table*}[!ht]

\centering % used for centering table
\resizebox{\textwidth}{!}{%
  \begin{tabular}{l c c c c c c c c c}
    %\thickhline 
    \toprule
    \multirow{2}{*}{\textbf{Model}} &
      \multicolumn{3}{c}{\textbf{DiffusionDB}} &
      \multicolumn{3}{c}{\textbf{Parti}} &
      \multicolumn{3}{c}{\textbf{DrawBench}} \\
      \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}%
    & ImageReward & Aesthetic & Human & ImageReward & Aesthetic & Human & ImageReward & Aesthetic & Human\\
    \midrule
    Stable V1.5 & 0.082  & \textbf{5.907}  & 25.6\% & 0.256  & 5.373 & 26.7\% & 0.001 & \textbf{5.229} & 31.2\% \\
    Stable V2 & 0.170 & 5.783 & 17.8\% & 0.414 & 5.269 & 25.3\% & 0.142 & 5.067 & 29.6\% \\
    ReFL  & \textbf{1.290} & 5.845 & 18.6\% &\textbf{0.832} & 5.402 & 35.4\% & \textbf{0.591} & 5.164 & 35.9\% \\
    RAFT & 0.338  & 5.881 & 17.7\% & 0.504 & \textbf{5.413} & 28.0\% & 0.303 & 5.185 & 35.7\% \\
    DRaFT & 0.818 & 5.645 & 18.9\% & 0.632 & 5.279 & 36.7\% &  0.338 & 5.079 & 42.0\% \\
    Reward-weighted & 0.438 & 5.821 & 22.4\% & 0.624 & 5.363 & 29.2\% & 0.456 & 5.148 & 30.6\% \\ \midrule
    Ours & \textbf{0.845} & \textbf{5.918} & --- & \textbf{0.731} & \textbf{5.477} & --- & \textbf{0.583} & \textbf{5.287}  & --- \\
    \bottomrule
  \end{tabular}%
}

\caption{\textbf{Quantitative Results.} ImageReward scores and Aesthetic scores from the original SD2 models, models trained with baseline fine-tuning methods including ReFL, RAFT, DRaFT and Reward-weighted training, as well as our RL fine-tuned model. We report the average ImageReward and Aesthetic scores across images generated from 2,000 prompts from DiffusionDB dataset. The images are generated using the same random seeds for all models for fair comparison.}

% \et{TBD: could be worth separating out the reward values from the human eval. probably good strategically to frontload the key result, and the discussion of the reward values can be deferred -> lead into the discussion of reward hacking
% there's also a weird mismatch with what these metrics mean}
% } % title of Table
% }
\label{table:imagereward_allbaselines} % is used to refer this table in the text
\end{table*}

